CeNTREX: A new search for time-reversal symmetry violation in the $^{205}$Tl nucleus

The Cold molecule Nuclear Time-Reversal EXperiment (CeNTREX) is a new effort aiming for a significant increase in sensitivity over the best present upper bounds on the strength of hadronic time reversal ($T$) violating fundamental interactions. The experimental signature will be shifts in nuclear magnetic resonance frequencies of $^{205}$Tl in electrically-polarized thallium fluoride (TlF) molecules. Here we describe the motivation for studying these $T$-violating interactions and for using TlF to do so. To achieve higher sensitivity than earlier searches for $T$-violation in TlF, CeNTREX uses a cryogenic molecular beam source, optical state preparation and detection, and modern methods of coherent quantum state manipulation. Details of the measurement scheme and the current state of the apparatus are presented, with quantitative measurements of the TlF beam. Finally, the estimated sensitivity and methods to control systematic errors are discussed.

==> figs/svg/Makefile <==
.PHONY: all clean

%.pdf: %.svg
	inkscape -D --export-latex --export-filename=$@ $<
	sed -i '' 's/$@/figs\/svg\/$@/g' $@_tex

all: lasers1.pdf lasers2.pdf beamline_to_state_prep_b.pdf

clean:
	rm -f *.pdf *.pdf_tex


==> rosetta_stone.tex <==
\section{Rosetta stone}
Compiling a list of symbols and their definitions. Not meant to be included in actual publication.

\subsection{Abbreviations}
\begin{itemize}
    \item Parts of experiment:
    \begin{itemize}
        \item BS = beam source
        \item RC = rotational cooling region
        \item SPA = state preparation region A
        \item EQL = electrostatic quadrupole lens
        \item SPB = state preparation region B
        \item MI = main interaction region
        \item SPC = state preparation region C
        \item FD = fluorescence detection region
    \end{itemize}
    
    \item Miscellaneous:
    \begin{itemize}
        \item EDM = electric dipole moment
        \item CPV = CP violation
        \item SM = Standard Model
        \item BAU = baryon asymmetry of the universe
        \item FCF = Franck-Condon factor
        \item NMR = nuclear magnetic resonance
        \item LIF = laser-induced fluorescence
        \item PMT = photomultiplier tube
        \item AP = adiabatic passage
        \item SOF = separated oscillatory fields
        \item MTS = modulation transfer spectroscopy
        \item NSM = nuclear Schiff moment
    \end{itemize}
    
\end{itemize}

\subsection{Coordinate systems}
\begin{itemize}
    \item Interaction region defines $\hat{z}$:
    \begin{itemize}
        \item $\hat{z}$ is defined by the direction of the electric field in the main interaction region
        \item $\hat{x}$ is along the direction of the molecular beam
        \item $\hat{y}$ is the remaining direction required to the define right-handed coordinate system
    \end{itemize}
    
    \item Molecular beam direction defines $\hat{Z}$:
        \begin{itemize}
        \item $\hat{Z}$ is defined by the average direction of the molecular beam. Also parallel to E-field in SPA.
        \item $\hat{Y}$ points up in the lab
        \item $\hat{X}$ is the remaining direction required to the define right-handed coordinate system
    \end{itemize}
    
    \item Rotating coordinate system: 
    \begin{itemize}
        \item $\hat{\zeta}$ is along direction of E-field at any given point along a molecule's trajectory
        \item $\hat{\xi}$ and $\hat{\upsilon}$ (equivalents of x and y) are not used 
    \end{itemize}
\end{itemize}

\subsection{Symbols}
\begin{itemize}
    \item Electric and magnetic fields:
    \begin{itemize}
        \item Scalar electric field: $\Esca$
        \item Vector electric field: $\Evec$
        \item Scalar magnetic field: $\Bsca$
        \item Vector magnetic field: $\Bvec$
    \end{itemize}
    \item CP violation parameters:
    \begin{itemize}
        \item $\bar{\theta}$ QCD CP-violating parameter 
    \end{itemize}
    \item Quantum numbers
    \begin{itemize}
        \item $J,\,m_J$: rotational quantum number
        \item $I_1,\,m_1$: Thallium nuclear spin
        \item $I_2\,m_2$: Fluoride nuclear spin
        \item $F_1 = J+I_1$: 
        \item $F = F_1 + I_2,\,m_F$: total angular momentum
        \item $\vec{\It} = \vec{I_1}+\vec{I_2},\, m_{\It}$: total nuclear spin
        \item $\widetilde{x}$: strongly mixed state where x denotes the relevant quantum number
        \item $x'$: excited state
    \end{itemize}
    \item TlF Schiff moment
    \begin{itemize}
        \item $S$: Schiff moment
        \item $\hat{\vec{n}}$: internuclear axis (points from F to Tl)
        \item ${\rm W}_{\rm S}$: size of energy shift for given SM
        \item $\mathcal{P}$: polarization
        \item $\widetilde{\Delta} = {\rm W}_{\rm S}S\mathcal{P}$: Schiff Moment energy shift
        \item $\left\langle \mathcal{H}_{CPV} \right\rangle = {\rm W}_{\rm S} S \mathcal{P} \frac{\Evec}{\Esca}\cdot\frac{\vec{I}}{I}$
    \end{itemize}
    \item Measurement
    \begin{itemize}
        \item $\phi$: total phase accumulation during free spin precession
        \item $\phi_{\rm SOF}$: phase offset between two SOF RF coils
        \item $\widetilde{\phi}$: phase accumulation during free spin precession due to the Schiff moment
        \item $\mathcal{A} = \frac{{\rm S}_\uparrow - {\rm S}_\downarrow}{{\rm S}_\uparrow + {\rm S}_\downarrow}$: measurement asymmetry, where ${\rm S}$ is the fluorescence signal.
    \end{itemize}
\end{itemize}
